Learning Deformable Tetrahedral Meshes for 3D Reconstruction

3D shape representations that accommodate learning-based 3D reconstruction are an open problem in machine learning and computer graphics. Previous work on neural 3D reconstruction demonstrated benefits, but also limitations, of point cloud, voxel, surface mesh, and implicit function representations. We introduce Deformable Tetrahedral Meshes (DefTet) as a particular parameterization that utilizes volumetric tetrahedral meshes for the reconstruction problem. Unlike existing volumetric approaches, DefTet optimizes for both vertex placement and occupancy, and is differentiable with respect to standard 3D reconstruction loss functions. It is thus simultaneously high-precision, volumetric, and amenable to learning-based neural architectures. We show that it can represent arbitrary, complex topology, is both memory and computationally efficient, and can produce high-fidelity reconstructions with a significantly smaller grid size than alternative volumetric approaches. The predicted surfaces are also inherently defined as tetrahedral meshes, thus do not require post-processing. We demonstrate that DefTet matches or exceeds both the quality of the previous best approaches and the performance of the fastest ones. Our approach obtains high-quality tetrahedral meshes computed directly from noisy point clouds, and is the first to showcase high-quality 3D tet-mesh results using only a single image as input. Our project webpage: https://nv-tlabs.github.io/DefTet/

==> source/applications_s.tex <==
\vspace{-4pt}
\section{Applications}
\label{sec:applications}
\vspace{-4pt}
We introduce our \ourmodel  to 3D reconstruction with either 3D or 2D supervision, and utilize differentiable loss functions to deform vertices and generate 3D objects.
\vspace{-4pt}
\subsection{3D reconstruction with 3D data}
\vspace{-4pt}
% We first introduce our algorithm to obtain occupancies and deform vertices when the 3D ground truth is available, and then show applications on tetrahedral meshing and point cloud 3D reconstruction.
\vspace{-4pt}
\paragraph{Occupancy:} We supervise the the occupancy prediction from $h$ with Binary Cross Entropy:
\begin{eqnarray}
L_{occ} = \sum_{k=1}^K \hat{O}_k \log (O_k) + (1-\hat{O}_k ) \log (1-O_k),
\end{eqnarray}
where $\hat{O}_k$ is the ground truth occupancy for tetrahedron $T_k$. We obtain $\hat{O}_k$ using winding number. In specific, for $T_k$, we first  obtain its geometric centroid by averaging its four vertices, and calculate its winding number with respect to the ground truth boundary mesh. If the winding number of the centroid of an tetrahedron is even, we consider the tetrahedron to be occupied, otherwise non-occupied. Note that, the occupancy of an tetrahedron is a piece-wise linear function of its four vertices, and thus, is dynamically changing when the tetrahedron is deforming. 
\vspace{-8pt}
\paragraph{Deformation:} With ground truth tetrahedron occupancy, we obtain the triangular faces whose visible probability equal to 1 using Eq.~\ref{eq:face_prob}. We denote them as $\mathcal{F}$. We deform $\mathcal{F}$ to align with the target object's surface, by minimizing the distances between two surface. In specific, we first sample a set of points $\mathcal{S}$ from the surface of the target object. For each sampled point, we minimize its distance to the closest face in $\mathcal{F}$. Besides, we also sample a set of points $\mathcal{S}_{\mathcal{F}}$ from $\mathcal{F}$, and minimize its distance to the closest points in $\mathcal{S}$:
\begin{eqnarray}
L_{\text{surf}} = \sum_{p\in \mathcal{S}} \min_{f\in\mathcal{F}} \text{dis}_f(p, f) + \sum_{q\in\mathcal{S}_{\mathcal{F}}} \min_{p\in\mathcal{S}} \text{dis}_p (p, q),
\end{eqnarray}
where $\text{dis}_f(p, f)$ is L2 distance from point $p$ to face $f$, and $\text{dis}_p (p, q)$ is L2 distance from point $p$ to $q$.
The overall loss function is:
\begin{eqnarray}
L_{\text{3D}} = L_{\text{occ}} + \lambda_{\text{surf}} L_{\text{surf}} + \lambda_{\text{reg}} L_{\text{reg}},
\end{eqnarray}
where $\lambda_{\text{surf}}$ and $\lambda_{\text{reg}}$ are hyperparamters. Note that all the loss functions are differentiable with respect to vertices' position and occupancy prediction, we could train neural network end-to-end.
\vspace{-4pt}
\subsubsection{Point Cloud 3D Reconstruction}
\label{sec:pc3d}
\vspace{-4pt}
We show application of our \ourmodel on reconstructing 3D shapes from noisy point cloud. Reconstruction from other input is also adaptable. We first adopt PointVoxel CNN~\cite{conv_occnet,pvcnn} to encode the input point cloud into a voxelized feature map. For each vertices, we grab the feature using trilinear interpolation and apply Graph-Convolutional-Network~\cite{curvegcn} to predict the deformation offset. For each tetrahedron, we use MLP to predict its centroid occupancy, whose feature is also obtained through trilinear interpolation using centroid position.  Architecture details are provided in Appendix.
\vspace{-4pt}
\subsubsection{Tetrahedral Meshing}
\vspace{-4pt}
Tetrahedral Meshing is a task to tetrahedralize the interior of a watertight boundary mesh~\cite{quartet,tetgen,tetwild}. Our \ourmodel can be applied to this task with two manners: optimization-based and learning-based. 
\vspace{-8pt}
\paragraph{Optimization-based:} We iteratively run two steps until obtain satisfactory result: 1) obtain the occupancy for each tetrahedron, 2) deform the tetrahedron by minimizing the $L_{\text{surf}} + \lambda_{\text{reg}}L_{\text{reg}} $ and back-propagate gradients to vertices' positions using gradient descent. 
% After optimization, we check the occupancy of each deformed tetrahedron and output the tetrahedron that lies inside of the object. 
\vspace{-4pt}
\paragraph{Learning-based:} To speedup the optimization, we first train a neural network proposed in Sec.~\ref{sec:pc3d} to learn the deformation offset, but takes in the clean point cloud as input. For the unseen shapes during inference, we first run prediction to get the initial offset, and further apply the optimization on previous paragraph to refine the prediction.

% \textbf{Laplacian}: neighboring point should have similar movement. \textbf{Volume}: all tetrahedron should have similar volume.  \textbf{Smoothness}: the normal of neighboring faces should have similar direction. \textbf{Delta:} the deformation for each point should be  small. 

% \begin{eqnarray}
% L_{\text{lap}} &=& \sum_v |\delta_v - \frac{1}{|\mathcal{N}|}\sum_{v^{\prime} \in \mathcal{N}} \delta_{v^{\prime}}|^2 \\
% L_{\text{volume}} &=& \frac{1}{M} \sum_{k=1}^M |V_k - \overline{V}|^4\\
%  L_{\text{normal}} &=& \sum (\mathbf{n}_{1} \cdot \mathbf{n}_{2} )^2\\
%  L_{\text{delta}} &=&n \sum_v |\delta_v|^2 \
% \end{eqnarray}






==> source/diffrender.tex <==
\iffalse
\vspace{-4pt}
\subsection{3D reconstruction with 2D data}
\vspace{-4pt}
%Recently, a branch of works have demonstrated that 3D objects could be learned from 2D supervision only. Their 3D representations range from voxel~\cite{drcTulsiani17} to mesh~\cite{dibr,softras,n3mr} or even SDF~\cite{}. Our deformable tetrahedron can also be supervised from 2D images, and avoid all the constraints in these representations we mentioned above.
To reconstruct 3D shape with 2D data, we design a novel differentiable rendering algorithm to project the deformable tetrahedron to a 2D image using the provided camera. We can even support per-vertex color and render an RGB image. 
\vspace{-4pt}
\paragraph{Differentiable Renderer:} Our \ourmodel can also be treated as a mesh, with a set of vertices $\mathbf{V}$ and faces $\mathbf{F}$. To render a RGB image with mask, we first assign or each vertex $v_i$ a RGB attribute $C_i$ and an visibility attribute $D_i$. For each pixel $I_j$, we shot a ray that starts from the camera origin, passes the pixel $I_j$ and hit some triangular faces in $\mathbf{F}$. Without loss of generality, we assume in total $\{f_{l_1}, \cdots, f_{l_L}\}$ are hit with $L$ being the total number, and they are sorted in the increasing order of the depth along the ray. We render all of these faces and softly combine them through visibility. 

For each hit face $f_{l_k}=(v_a, v_b, v_c)$, its attribute in the pixel $I_j$ is obtained with barycentric interpolation:
\begin{equation}
\begin{aligned}
w_a, w_b, w_c &= \text{Barycentric}(v_a, v_b, v_c, I_j) \\
D_j^k = w_aD_a + w_b&D_b + w_cD_c;  \quad  C_j^k = w_aC_a + w_bC_b + w_cC_c
\end{aligned}
\end{equation}
Inspired from volume rendering~\cite{nerf,sitzmann2019scene}, we propose that the visibility $m_k$ of face $f_{l_k}$ in pixel $I_j$ depends on its own visibility and all the faces in front of it. Namely, if all its front faces are not visible, then this face is visible: 
\begin{eqnarray}
m_k = \prod_{i=1}^{k-1}(1-D_j^i)D_j^k
\end{eqnarray}
Finally, we use weighted sum to obtain the color $R_j$ and visibility $M_j$ for pixel $I_j$ as below:
\begin{equation}
\begin{aligned}
M_j = \sum_{k=1}^{L}m_{k}; \quad R_j &= \sum_{k=1}^{L}m_{k}C_{j}^k
\end{aligned}
\end{equation}
Note that the gradients from $M_j$ and $R_j$ can be naturally back propogated to not only color and visibility attributes, but also vertex positions via barycentric weights based on chain rules. 
\vspace{-4pt}
\paragraph{Occupancy:} For each tetraedron, we empirically find using the max over its four vertices as its occupancy: $O_k = \max(D_{a_k}, D_{b_k}, D_{c_k}, D_{d_k})$ is the best.
\vspace{-4pt}
\paragraph{Loss functions:}
We use the L1 distance between the rendered image and ground truth image to supervise the network:
\begin{equation}
\begin{aligned}
L_{\text{2D}} = \sum_{j}^{}\left | R_{j}^{GT} - R_j \right |_1  + \left| M_{j}^{GT} - M_j \right |_1
\end{aligned}
\end{equation}
\fi


% Our \ourmodel can also be treated as a mesh, with a set of vertices $\mathbf{V}$ and faces $\mathbf{F}$, where many faces can cover one pixel in an image, as shown in Fig.~\ref{}. We first assign each vertex $v_i$ a RGB attribute $C_i$ and an occupancy attribute $O_i$. If a face $f=(v_a, v_b, v_c)$ covers the pixel $I_j$, we can render the pixel using barycentric interpolation, as:
% \begin{equation}
% \begin{aligned}
% w_a, w_b, w_c &= \text{Barycentric}(v_a, v_b, v_c, I_j) \\
% O_j = w_aO_a + w_b&O_b + w_cO_c  \quad  C_j = w_aC_a + w_bC_b + w_cC_c
% \end{aligned}
% \end{equation}
% Now imagine that a ray starts from camera origin, passes the pixel $I_j$ and hit many faces. While traditional rendering only draws the most front face, instead we draw all the faces that would cover $I_j$, as shown below:
% \begin{eqnarray}
% (o_1, c_1), (o_2, c_2), & ..., (o_n, c_n) = R(V, F, I_j)
% \end{eqnarray}
% Since the light passes front faces first, we assume that all the drawing $(o_1, c_1), (o_2, c_2),  \cdots, (o_n, c_n)$ are sorted by face depth. We then consider how to merge them into one pixel value. Inspired by ray tracing~\cite{} and volume rendering~\cite{}, we propose that the visibility of face $k$, where we refer to $m_k$, depends on its own occupancy $o_k$ and all the faces in front of it. Namely, if all its front faces are not visible, then this face is visible: 
% \begin{eqnarray}
% m_k = \prod_{i=1}^{k-1}(1-o_i)o_k
% \end{eqnarray}
% Finally, we simply adopts weighted sum to calculate the color $C_j$ and occupancy $M_j$ for pixel $I_j$ as below. Note that in this way the image gradients can be naturally back propogated to color attributes and occupancy attributes. Moreover, based on chain rules, the gradients can also be passed to vertex positions via barycentric weights.
% \begin{equation}
% \begin{aligned}
% M_j = \sum_{i=1}^{n}m_{i} \quad C_j &= \sum_{i=1}^{k}m_{i}c_{i}
% \end{aligned}
% \end{equation}

% \paragraph{Loss functions:}


% Since a tetrahedron coule be rendered into a image in a differentiable way, thus we can also optimize a tetrahedron, adjusting its vertex positions, RGB and occupancy attributes $V, C, O$, totally from 2D supervision. That's to say, given 2D images, we seek the optimal $V^*, C^*, O^*$ to minimize the $N$ pixel loss between the GT and the rendering, where:

% \begin{equation}
% \begin{aligned}
% L_{2D} = \frac{1}{N}\sum_{j=1}^{N}\left | I_{j}^{GT} - R(V, F, I_j) \right |_1 \quad V^*, C^*, O^* = argmin_{V, O, C} L_{2D} 
% \end{aligned}
% \end{equation}

% We then clip the invisible tetrahedron and convert it into a mesh. \wz{where is the definition of $T$ in 3D?}.



%\subsection{3D Tetrahedral Meshing from 2D Supervision}

%\subsection{Single Image 3D Reconstruction from 2D Supervision}

==> source/next.tex <==
\section{Next directions}

